A Multi-In and Multi-Out Dendritic Neuron Model and its Optimization

Artificial neural networks (ANNs), inspired by the interconnection of real neurons, have achieved unprecedented success in various fields such as computer vision and natural language processing. Recently, a novel mathematical ANN model, known as the dendritic neuron model (DNM), has been proposed to address nonlinear problems by more accurately reflecting the structure of real neurons. However, the single-output design limits its capability to handle multi-output tasks, significantly lowering its applications. In this paper, we propose a novel multi-in and multi-out dendritic neuron model (MODN) to tackle multi-output tasks. Our core idea is to introduce a filtering matrix to the soma layer to adaptively select the desired dendrites to regress each output. Because such a matrix is designed to be learnable, MODN can explore the relationship between each dendrite and output to provide a better solution to downstream tasks. We also model a telodendron layer into MODN to simulate better the real neuron behavior. Importantly, MODN is a more general and unified framework that can be naturally specialized as the DNM by customizing the filtering matrix. To explore the optimization of MODN, we investigate both heuristic and gradient-based optimizers and introduce a 2-step training method for MODN. Extensive experimental results performed on 11 datasets on both binary and multi-class classification tasks demonstrate the effectiveness of MODN, with respect to accuracy, convergence, and generality.

==> paper/backup/conclusion.tex <==
\section{Conclusion}\label{con}
In this study, we propose a novel multi-output dendritic neuron model for solving multi-class classification problems. Instead of stacking multiple DNMs, our model utilizes a preference filter to select the dendrites for maximum use the learnabel information in data. Meanwhile, we also provide two especial models, MODNP and MODNF, with two fixed preference filter, respectively. Specially, MODNP is nearly equivalent to multiple single-output neurons. Additionally, we design the telodendron layer to process the multiple outputs. Furthermore, our model based on BP is prone to ``dendrite dying'' and falling into local optimal solutions. Therefore, we use seven heuristic algorithms to optimize the model in order to obtain more stable and better performance. Then, extensive experiments verify BBO is currently the most effective optimization algorithm and MODNF presents MODNF is generally better than MLP and DNM. Our framework presents a new perspective for the foundation struction of neural networks. we will extend it to deeper and larger network models to handle more complex tasks.

==> paper/backup/experiment.tex <==
\section{Experiments}\label{experiments}

\begin{table*}[htb]
\centering
\caption{Detailed descriptions of the classification datasets}
\label{table1}
\begin{tabular}{cccccc}
\toprule
\textbf{Dataset}              & \textbf{Num. of training samples} & \textbf{Num. of testing samples} & \textbf{Num. of classes} & \textbf{Dimensionality} & \textbf{Explanation}                 \\ \hline
Breast cancer        & 546                      & 137                     & 2               & 9              & benign or malignant         \\
Blood transfusion    & 598                      & 150                     & 2               & 4              & donate blood or not         \\
Heart disease        & 212                      & 91                      & 2               & 13             & angiographic disease status \\
Raisin grains        & 720                      & 180                     & 2               & 7              & varieties of raisin         \\
Caesarian Section    & 64                       & 16                      & 2               & 5              & recommend cesarean or not   \\
Glass identification & 171                      & 43                      & 6               & 9              & types of glasses            \\
Wine                 & 142                      & 36                      & 3               & 13             & types of wines              \\
Car evaluation       & 1209                     & 519                     & 4               & 6              & car acceptability           \\
Iris                 & 90                       & 60                      & 4               & 4              & types of iris               \\
Seeds                & 168                      & 42                      & 3               & 7              & varieties of wheat          \\
Ecoli                & 228                      & 99                      & 5               & 7              & protein localization sites  \\ \bottomrule
\end{tabular}
\end{table*}

In this section, not only do we evaluate and analyze our three types of method with different optimized methods on eleven benchmark datasets, but our model are compared with the traditional MLP and DNM on binary classification and multi-class classification tasks. Especially, we use a mean result of 30 times for each experiment as an evaluation indicator.
\subsection{Datasets and implementation details}
\noindent \textbf{Datasets.} We experiment on the following five binary classification datasets: Breast cancer \cite{breast}, Blood transfusion \cite{blood}, Heart disease\cite{heart}, Raisin grains \cite{ccinar2020classification}, and Caesarian Section \cite{caesarian}. Additionally, we use six multi-class classification datasets: Glass identification \cite{glass}, Wine \cite{wine}, Car evaluation \cite{car}, Iris \cite{iris}, Seeds \cite{seeds} and Ecoli \cite{ecoli} to further confirm the capability of our method in handling multi-class classification tasks. All the above mentioned datasets for both binary and multi-class classifications are directly taken from University of California \cite{blake1998uci}. We manually create our own train/test data split since they are not officially provided in all of these datasets. The details for each dataset are summarized in Tab. \ref{table1}.

\begin{table}
\caption{Parameters of the optimization algorithms}
\label{table2}
\begin{tabular}{lll}
\toprule
\textbf{Method} & \textbf{Parameter}                      & \textbf{Option}                                                                                                \\ \hline
BP     & learning rate                  & 0.01                                                                                                 \\
       & maximum iterations $R$            & 3000                                                                                                 \\
BBO    & modification probability       & 1                                                                                                    \\
       & immigration probability bounds & {[}0, 1{]}                                                                                           \\
       & step size                      & 1                                                                                                    \\
       & maximum immigration rate       & 1                                                                                                    \\
       & maximum migration rate         & 1                                                                                                    \\
       & mutation probability           & 0.1                                                                                                  \\
       & population size                & 100                                                                                                  \\
       & maximum iterations $R$            & \begin{tabular}[c]{@{}l@{}}300 for Breast, Blood, Wine, \\ Car and Iris; 400 for others\end{tabular} \\
GA     & encoding strategy              & binary gray                                                                                          \\
       & crossover probability          & 1                                                                                                    \\
       & mutation probability           & 0.01                                                                                                 \\
       & population size                & 100                                                                                                  \\
       & maximum iterations $R$            & \begin{tabular}[c]{@{}l@{}}300 for Breast, Blood, Wine, \\ Car and Iris; 400 for others\end{tabular} \\
PSO    & inertia weight                 & 1                                                                                                    \\
       & cognitive coefficient          & 0.3                                                                                                  \\
       & social coefficient             & 0.3                                                                                                  \\
       & population size                & 200                                                                                                  \\
       & maximum iterations $R$            & \begin{tabular}[c]{@{}l@{}}300 for Breast, Blood, Wine, \\ Car and Iris; 400 for others\end{tabular} \\
PBIL   & learning rate                  & 0.05                                                                                                 \\
       & negative learning rate         & 0.05                                                                                                 \\
       & num. of best individuals       & 1                                                                                                    \\
       & num. of bad populations        & 0                                                                                                    \\
       & population size                & 200                                                                                                  \\
       & maximum iterations $R$            & \begin{tabular}[c]{@{}l@{}}300 for Breast, Blood, Wine, \\ Car and Iris; 400 for others\end{tabular} \\
ES     & global variance                & 1                                                                                                    \\
       & num. of new individuals        & 10                                                                                                   \\
       & population size                & 250                                                                                                  \\
       & maximum iterations $R$            & \begin{tabular}[c]{@{}l@{}}300 for Breast, Blood, Wine, \\ Car and Iris; 400 for others\end{tabular} \\ \bottomrule
\end{tabular}
\end{table}

\noindent \textbf{Implementation details.} Our model involves three key hyperparameters: dendrite number $M$, synaptic scaling factor $\alpha_{s}$, and telodendron scaling factor $\alpha_{t}$. Since we notice that the classification performance is sensitive to these three hyperparameters, we carefully tune them on each dataset to hopefully achieve the best classification accuracy. See Sec. \ref{statis} for a detailed ablation. The parameter settings for each optimization algorithm are listed in Tab. \ref{table2}. For all the heuristic algorithms, we directly adopt the originally provided configurations from the corresponding literature or the open source library \footnote{Available from http://geatpy.com/index.php/home/}. All the quantitative evaluations in following of this section report the averaged
experimental results for 30 runs to respect the criterion of significance test. 

\subsection{Quantitative evaluation} \label{evaluation}
We first investigate the performance of three types of our MODN under six types of optimization strategies. To provide a deeper understanding, we also assess two variants of MODN, namely MODNP and MODNF. Tab. \ref{table3} shows the classification results. It can be observed that among all the optimization methods, BBO achieves the superior performance on most datasets (9 in 11), whereas BP is generally less capable of exploring a decent optimization. The main reason is that, while resetting the 0 gradients to 1 eases the dilemma of "dendrite dying" for BP, the multiplication operation in Eqs. \ref{eq:eq15} to \ref{eq:eq18} can still result in excessively small gradients. Further, naively adopting a larger multiplier to amplify the gradients would by contrast destroy the required gradient update rule, \gu{as shown in xx.} 

To gain more insights into our model variants, we introduce the average sort score (\textbf{ASS}) to inspect the performance of stabilization on each dataset. To do so, for the $j$-th optimization method, we first sort each model based on the classification performance in descending order (e.g., the best model is sorted in the first), and then score each model with the corresponding order with $s_{j}$. The ASS is eventually calculated by averaging the score on all $J$ types (equals to 6 in our experiment) of optimization methods, which is given by $\rm{ASS} = \sum_{j}s_j/J$. The final column of Tab. \ref{table3} shows the ASS score. We can see that MODNF generally achieves the most stable learning effectiveness on all datasets (8 in 11). Based on these observation, we select the BBO algorithm for optimization, and MODNF framework for classification learning in the following sections.
% In this section, at first, we evaluate three types of our model with six optimization algorithms to explore and analyse which variant is outstanding on eleven datasets. More clearly, we select a stabilized variant on basis of the average sort score (ASS), which is computed from the average sort of the three frameworks using different optimization algorithms on every datasets. The results of performance and sort are reported in Tab. \ref{table3}. We can find from Tab. \ref{table3} that BBO algorithm is the most effective one to explore the optimal solution compared to others on nearly all of datasets. 
%Moreover, the reason for which the most popular BP is the worst way is the gradient is no longer updated in the dying dendrites. While all 0 gradients are forced to be 1 can ease the dilemma of the 0 gradient, the performance does not get any better because of the partial derivative $Z_{j}$ with respect to $Y_{ij}$ in Eq. \ref{eq:eq15} to \ref{eq:eq18} formulated by a multiplicative function is nearly 0. In a word, heuristic algorithms are more effective than gradient-based algorithms for optimizing our model. As can observed in the final column of Tab. \ref{table3}, we notice that MODN does not always perform the best on most datasets. We assume the reason is altering the elements in matrix $\textbf{P}$ to 0 will deactivate the parameters in the corresponding dendrites during the processing of training. The temporarily deactivated dendrite will not update following the correct direction until it is reactivated. The results in Tab. \ref{table3} evidence that MODN underperforms its two special states, MODNP and MODNF. We further observe that MODNF is sightly better than MODNP. To summarize, we select the MODNF framework and BBO algorithm as our mainstream and optimization strategy for follow-up experiments.

\begin{table*}
\centering
\caption{The results between three types of our model with six optimization strategies}
\label{table3}
\scalebox{1.2}{
\begin{tabular}{{lccccccc:c}}
\toprule
 & & \textbf{BBO} & \textbf{BP} & \textbf{GA} & \textbf{PSO} & \textbf{PBIL}  & \textbf{ES}   & \textbf{ASS} \\ \hline
\multirow{3}{*}{Breast cancer} & MODN   & 0.7402          & -      & 0.7411 & 0.7400 & 0.7409 & 0.7364 & 2.20          \\
                               & MODNP  & 0.7740          & 0.4680 & 0.7300 & 0.7402 & 0.7460 & 0.7358 & 2.17          \\
                               & MODNF  & \textbf{0.7953} & 0.5844 & 0.7358 & 0.7436 & 0.7387 & 0.7393 & \textbf{1.50} \\ \hdashline
\multirow{3}{*}{Blood transfusion} & MODN  & 0.6560          & -      & 0.7452 & 0.9319 & 0.9112 & 0.7277 & 2.40          \\
                                   & MODNP & \textbf{0.9781} & 0.5178 & 0.7134 & 0.8233 & 0.8567 & 0.7961 & 2.17          \\
                                   & MODNF & 0.9766          & 0.5275 & 0.7706 & 0.9613 & 0.9333 & 0.7815 & \textbf{1.33} \\ \hdashline
\multirow{3}{*}{Heart disease} & MODN  & 0.6703          & -      & 0.6703 & 0.6802 & 0.6824 & 0.6703 & 2.20          \\
                              & MODNP & 0.7066          & 0.4659 & 0.6718 & 0.6703 & 0.6788 & 0.6703 & 2.00          \\
                              & MODNF & \textbf{0.7201} & 0.4545 & 0.6729 & 0.6824 & 0.6941 & 0.6703 & \textbf{1.67} \\ \hdashline
\multirow{3}{*}{Raisin grains} & MODN   & 0.6144          & -      & 0.6461 & 0.8122 & 0.8033 & 0.6216 & 2.20          \\
                               & MODNP  & 0.8365          & 0.5122 & 0.6444 & 0.8022 & 0.7722 & 0.6770 & 2.33          \\
                               & MODNF  & \textbf{0.8376} & 0.5431 & 0.6661 & 0.8300 & 0.8009 & 0.6756 & \textbf{1.33} \\ \hdashline
\multirow{3}{*}{Caesarian section} & MODN   & 0.4146 & -      & 0.5750 & 0.6479 & 0.6229          & 0.3896 & 2.60          \\
                                   & MODNP  & 0.5604 & 0.4104 & 0.6250 & 0.6271 & \textbf{0.6708} & 0.3917 & 1.67          \\
                                   & MODNF  & 0.5688 & 0.4646 & 0.6146 & 0.6062 & 0.6646          & 0.4188 & \textbf{1.40} \\ \hdashline
\multirow{3}{*}{Glass identification} & MODN   & 0.3566          & -      & 0.2969 & 0.3302 & 0.3287 & 0.3287 & 2.00          \\
                                      & MODNP  & 0.3829          & 0.2821 & 0.2922 & 0.2992 & 0.2922 & 0.3202 & 2.33          \\
                                      & MODNF  & \textbf{0.4651} & 0.1876 & 0.3008 & 0.3566 & 0.3310 & 0.3194 & \textbf{1.50} \\ \hdashline
\multirow{3}{*}{Wine} & MODN   & 0.4380          & -      & 0.2778 & 0.4685 & 0.4278 & 0.4509 & \textbf{1.60} \\
                      & MODNP  & \textbf{0.6769} & 0.3519 & 0.2694 & 0.4305 & 0.3676 & 0.4398 & 2.33          \\
                      & MODNF  & 0.6537          & 0.3028 & 0.2759 & 0.5185 & 0.4231 & 0.4463 & 1.83          \\ \hdashline
\multirow{3}{*}{Car evaluation} & MODN   & 0.7071          & -      & 0.7065 & 0.7222 & 0.7160 & 0.7067 & 2.40          \\
                                & MODNP  & \textbf{0.7975} & 0.2453 & 0.7114 & 0.7216 & 0.7200 & 0.7074 & 1.83          \\
                                & MODNF  & 0.7440          & 0.3801 & 0.7129 & 0.7184 & 0.7177 & 0.7084 & \textbf{1.67} \\ \hdashline
\multirow{3}{*}{Iris} & MODN   & 0.6028          & -      & 0.6011 & 0.8361 & 0.7422 & 0.5300 & 2.40          \\
                      & MODNP  & \textbf{0.9433} & 0.3072 & 0.6111 & 0.8667 & 0.7728 & 0.5128 & \textbf{1.33} \\
                      & MODNF  & 0.7556          & 0.2800 & 0.5806 & 0.6917 & 0.6711 & 0.6528 & 2.33          \\ \hdashline
\multirow{3}{*}{Seeds} & MODN   & 0.5095          & -      & 0.4302 & 0.6833 & 0.5929 & 0.5437 & 2.80          \\
                       & MODNP  & \textbf{0.9286} & 0.3810 & 0.5095 & 0.6865 & 0.6952 & 0.5889 & \textbf{1.33} \\
                       & MODNF  & 0.7540          & 0.4286 & 0.5246 & 0.6341 & 0.6246 & 0.5540 & 1.83          \\ \hdashline
\multirow{3}{*}{Ecoli} & MODN   & 0.3559 & -      & 0.3566 & 0.5003 & 0.4696 & \textbf{0.6865} & 2.20          \\
                       & MODNP  & 0.5710 & 0.2737 & 0.3623 & 0.4121 & 0.4552 & 0.6581          & 2.00          \\
                       & MODNF  & 0.4700 & 0.2296 & 0.3848 & 0.5081 & 0.4875 & 0.3694          & \textbf{1.67} \\ \bottomrule
\end{tabular}}
\end{table*}

\begin{figure}
\centering
\subfloat[Breast]{\label{fig3:a}\includegraphics[width=0.45\linewidth]{paper/figure/experiment/loss/breast_com.pdf}}\quad
\subfloat[Blood transfusion]{\label{fig3:b}\includegraphics[width=0.45\linewidth]{paper/figure/experiment/loss/blood-transfusion_com.pdf}}\\
\subfloat[Car]{\label{fig3:c}\includegraphics[width=0.45\linewidth]{paper/figure/experiment/loss/car_com.pdf}}\quad
\subfloat[Iris]{\label{fig3:d}\includegraphics[width=0.45\linewidth]{paper/figure/experiment/loss/iris_com.pdf}}\\
\caption{The performance with three different parameters on the Raisin and Iris}
\label{fig:3}
\end{figure}

\subsection{Comparison against other methods} 
We here quantitatively evaluate the classification performance of our model against prior methods. Specifically, we compare with two baseline artificial neural network models: MLP and DNM \cite{gao2019dendritic}. Since we focus on investigating the performance under shallowly-structured models, we create a 2-layer MLP for fair comparisons. The hidden layer dimensionality for MLP is set with the dendrite number $M$ to be consistent with our model. Also, the MLP is optimized via the same loss function (i.e., cross-entropy) with its final output layer designed as a softmax activation, as ours. As for DNM, we set $(\alpha_{t}, \alpha_{s})$ as the same value as ours for all datasets considering the structure resemblance. We use the fine-tuned value of $\theta$ for DNM as suggested in \cite{gao2019dendritic}. All the hyperparameters of our model (after fine-tuning) are listed in Tab. \ref{table4}. 

\noindent \textbf{Evaluation metrics.} The overall performance evaluation is measured with the average accuracy (\textbf{ACC}) and area under the ROC curve (\textbf{AUC}) metrics over 30 runs. ACC is calculated by $\rm{ACC} = \sum_{n=1}^{N}\mathbb{I}(\widehat{O}^n = \tau(O^n))$, in which $\tau(\cdot)$ is a mapping that one-hot vectorizes our network output $O^n$, and $\mathbb{I}(\cdot)$ is the indicator function. Then, AUC is calculated by the confusion matrix composed of true positive (TP), true negative (TN), false positive (FP) and false negative (FN). TP and TN present the number of correctly classified positive and negative samples, respectively. FP refers to the number of positive samples incorrectly classified, whereas FN refers to the negative samples labeled correctly. In terms of binary classification, for any selected positive class, we calculate the true positive rate (\textbf{TPR}, also termed as recall), via $\rm{TPR = TP/(TP+FN)}$, and the false positive rate (\textbf{FPR}) via $\rm{FPR = FP/(FP+TN)}$. While for multi-class classification, we follow the micro-averaging policy by deriving \textbf{TPR} and \textbf{FPR} with $\rm{TPR} = \sum_c\rm{TP}_c/ \sum_c(\rm{TP}_c+\rm{FN}_c)$ and $\rm{FPR} = \sum_c\rm{FP}_c/ \sum_c(\rm{FP}_c+\rm{TN}_c)$, where $c \in \mathcal{C}$ is the assumed one positive class, leaving the rest classes to be negative. The obtained TRPs and FPRs for both binary and multi-class cases are then respectively set to y- and x-axises to plot the ROC curve. 

To further systematically evaluate the performance of all three methods, we adopt the Wilcoxon signed-rank test (WSRT) \cite{garcia2009study} as an assessment criteria of significant difference between ours and the compared models. Assume, in the $i$-th run, the paired experimental results (ACC) of two methods (i.e., one for ours and the other for the compared model) for WSRT are $A_i^1$ and $A_i^2$. WSRT calculates a positive-negative signed-rank sum pair ($\mathbf{W^{+}}, \mathbf{W^{-}}$) as the test statistic via 


%While for multi-class classification, we use the micro-averaging to aggregate the value from every class and regard the rest classes as the negative class for each class. The formulas of TPR and FPR can be written by $\rm{TPR} = \sum_c\rm{TP}_c/ \sum_c(\rm{TP}_c+\rm{FN}_c)$ and $\rm{FPR} = \sum_c\rm{FP}_c/ \sum_c(\rm{FP}_c+\rm{TN}_c)$. 
\begin{equation}
\label{eq:eq23}
\left\{
\begin{aligned}
\mathbf{W^{+}}=\sum_{i=1}^{30}sgn(A_i^2-A_i^1)R_{i}  \quad  if A_i^2-A_i^1>0, \\
\mathbf{W^{-}}=\sum_{i=1}^{30}sgn(A_i^2-A_i^1)R_{i}  \quad  if A_i^2-A_i^1<0,
\end{aligned}
\right.
\end{equation}
where $R_{i}$ indicates the rank of the absolute value of the difference between $A_i^2$ and $A_i^1$, and $sgn()$ denotes the sign function. Note that in the case that the difference of two paired samples are equal, the ranks computed in both runs will be re-assigned with the averaged ranks. Also, if $A_i^1$ is equal to $A_i^2$, then the result pair (both $A_i^1$ and $A_i^2$) will be removed from the rank calculation. 
After obtaining ($\mathbf{W^{+}}, \mathbf{W^{-}}$), WSRT computes the final statistic $-$ p-value as the significance indicator. Considering the high sample size, we use normal distribution approximation for calculation. In particular, we follow the standard WSRT protocols by first estimating the Gaussian parameters via $\hat{\mu} = T(T+1)/4$ and $\hat{\delta} = \sqrt{T(T+1)(2T+1)/24}$, where $T$ refers to the number of sample pairs with non-zero differences. Then, p-value $p$ can be derived by computing $p = P(X \leq \rm{min}\{\mathbf{W^{+}}, \mathbf{W^{-}}\})$, where $ X \sim \mathcal{N}(\hat{\mu},\hat{\delta}^2)$. Theoretically, a p-value smaller than 0.05 represents the difference between two compared methods  is significant at the 0.05 level. Besides, a larger $\mathbf{W^{+}}$ and a smaller $\mathbf{W^{-}}$ can also serve as the reference of significance.

%After obtaining ($\mathbf{W^{+}}, \mathbf{W^{-}}$), we use a normal approximation to compute p-value due to high sample size. The mean and variance can be estimated by $\hat{\mu} = T(T+1)/4$ and $\hat{\delta} = \sqrt{T(T+1)(2T+1)/24}$, where $T$ refers to the number of sample pairs with non-zero differences. Then, p-value can be estimated by $p = P(X \leq \rm{min}\{\mathbf{W^{+}}, \mathbf{W^{-}}\}| X \mathtt{\sim} N(\hat{\mu},\hat{\delta}^2))$. Theoretically, a p-value smaller than 0.05 represent the different between two methods compared is significant at the 0.05 level.

\gu{above from here is revised}
The quantitative results are reported in Tab. \ref{table5}. It can be confirmed that our model outperforms MLP by a large margin in all datasets (i.e., both tasks) with respect to AUC and ACC (Tab. \ref{table5} 3rd and 4th columns). The reason can be attributed to the fact that dendrite neural families intrinsically involve a mathematically modeled synapse layer that is capable of addressing the XOR problem. As for DNM, we can observe DNM is hard to deal with class imbalanced datasets (i.e. Breast cancer, Blood transfusion). 
%The preference filter can retain the special feature (via exclusive dendrites) from small samples in favor of imbalanced classification.
Compared DNM, the telodendron layer in our model can map every sample into a larger discriminative region via dividing into activated multiple branches.

%Furthermore, regarding the p-value (Tab. \ref{table5} last columns), we can observe that it is generally smaller than $10^{-6}$, which reflects the reliability of 

%and generally better than DNM on the binary classification task.

All of the evaluation results are reported in Tab. \ref{table5} and the ROC curve are shown in FIG. \ref{fig:3}. From the results, our model is significantly outperforms MLP on all tasks and generally better than DNM on the binary classification task.


\begin{table}
\centering
\caption{Tuned hyperparameter of MODNF in all classification datasets}
\label{table4}
\begin{tabular}{lccc}
\toprule
\textbf{Dataset} & $\mathbf{M}$ & $\mathbf{\alpha^s}$ & $\mathbf{\alpha^t}$ \\ \hline
Breast cancer        & 24       & 8                   & 1.5 \\
Blood transfusion    & 32       & 10                  & 1   \\
Heart disease        & 48       & 8                   & 1.5 \\
Raisin grains        & 8        & 5                   & 1   \\
Caesarian Section    & 16       & 1                   & 0.9 \\
Glass identification & 55       & 10                  & 1   \\
Wine                 & 28       & 10                  & 1   \\
Car evaluation       & 32       & 10                  & 1   \\
Iris                 & 12       & 5                  & 1   \\
Seeds                & 16       & 10                  & 1   \\
Ecoli                & 30       & 10                  & 1   \\ \bottomrule
\end{tabular}
\end{table}

\begin{table*}
\centering
\caption{The result}
\label{table5}
\begin{tabular}{llccccc}
\toprule
\textbf{Datasets}                     & \textbf{Methods}  & \textbf{AUC}$\uparrow$    & \textbf{ACC}$\uparrow$    & $\mathbf{W^{+}}\uparrow$ & $\mathbf{W^{-}}\downarrow$ & \textbf{p-value (0.05)$\downarrow$} \\ \hline
\multicolumn{7}{c}{\textbf{Binary classification}} \\ \hline
\multirow{3}{*}{Breast cancer}        & MLP          & 0.8364          & 0.8397          & 465.0       & 0.0         & \underline{1.862645e-09}     \\
                                      & DNM          & 0.9966          & 0.9824          & 183.5       & 92.5        & 1.648645e-01     \\
                                      & MODNF (ours) & \textbf{0.9984} & \textbf{0.9854} & -           & -           & -                \\ \hdashline
\multirow{3}{*}{Blood transfusion}    & MLP          & 0.7660          & 0.7393          & 465.0       & 0.0         & \underline{2.502268e-06}     \\
                                      & DNM          & 0.7532          & 0.7860          & 311.0       & 67.0        & \underline{3.431032e-03}     \\
                                      & MODNF (ours) & \textbf{0.8479} & \textbf{0.7967} & -           & -           & -                \\ \hdashline
\multirow{3}{*}{Heart diease}         & MLP          & 0.6011          & 0.6612          & 464.0       & 1.0         & \underline{3.725290e-09}     \\
                                      & DNM          & \textbf{0.9063} & 0.7853          & 327.0       & 108.0       & \underline{1.828005e-02}     \\
                                      & MODNF (ours) & 0.9031          & \textbf{0.8147} & -           & -           & -                \\ \hdashline
\multirow{3}{*}{Raisin grains}        & MLP          & 0.6645          & 0.5854          & 434.0       & 1.0         & \underline{2.979178e-06}     \\
                                      & DNM          & \textbf{0.9426} & \textbf{0.8793} & 0.0         & 435.0       & \underline{2.687907e-06}     \\
                                      & MODNF (ours) & 0.9103          & 0.8489          & -           & -           & -                \\ \hdashline
\multirow{3}{*}{Caesarian section}    & MLP          & 0.4978          & 0.4521          & 435.0       & 0.0         & \underline{2.289248e-06}     \\
                                      & DNM          & \textbf{0.7189} & 0.5479          & 378.0       & 0.0         & \underline{5.417129e-06}     \\
                                      & MODNF (ours) & 0.6853          & \textbf{0.7271} & -           & -           & -                \\ \hline
\multicolumn{7}{c}{\textbf{Multi-class classification}} \\ \hline
\multirow{2}{*}{Glass identification} & MLP          & 0.6312          & 0.2930          & 434.0       & 1.0         & \underline{2.971257e-06}     \\
                                      & MODNF (ours) & \textbf{0.8439} & \textbf{0.4775} & -           & -           & -                \\ \hdashline
\multirow{2}{*}{Wine}                 & MLP          & 0.7151          & 0.5389          & 372.0       & 63.0        & \underline{8.612798e-04}     \\
                                      & MODNF (ours) & \textbf{0.8442} & \textbf{0.6601} & -           & -           & -                \\ \hdashline
\multirow{2}{*}{Car evaluation}       & MLP          & 0.7842          & 0.6683          & 90.0        & 1.0         & 4.399668e-01     \\
                                      & MODNF (ours) & \textbf{0.9176} & \textbf{0.7439} & -           & -           & -                \\ \hdashline
\multirow{2}{*}{Iris}                 & MLP          & 0.6349          & 0.4117          & 435.0       & 0.0         & \underline{2.693323e-06}     \\
                                      & MODNF (ours) & \textbf{0.9345} & \textbf{0.7906} & -           & -           & -                \\ \hdashline
\multirow{2}{*}{Seeds}                & MLP          & 0.6882          & 0.4944          & 430.0       & 5.0         & \underline{4.509593e-06}     \\
                                      & MODNF (ours) & \textbf{0.9587} & \textbf{0.8087} & -           & -           & -                \\ \hdashline
\multirow{2}{*}{Ecoli}                & MLP          & 0.5657          & 0.2872          & 406.0       & 0.0         & \underline{3.977420e-06}     \\
                                      & MODNF (ours) & \textbf{0.8154} & \textbf{0.4845} & -           & -           & -                \\ \bottomrule
\end{tabular}
\end{table*}


\begin{figure*}
\centering
\subfloat[Breast]{\label{fig4:a}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/breast_roc.pdf}}\quad
\subfloat[Blood transfusion]{\label{fig4:b}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/blood-transfusion_roc.pdf}}\quad
\subfloat[Heart]{\label{fig4:c}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/heart_roc.pdf}}\quad
\subfloat[Raisin]{\label{fig4:d}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/raisin_roc.pdf}}\\
\subfloat[Caesarian]{\label{fig4:e}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/caesarian_roc.pdf}}\quad
\subfloat[Glass]{\label{fig4:f}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/glass_roc.pdf}}\quad
\subfloat[Wine]{\label{fig4:g}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/wine_roc.pdf}}\quad
\subfloat[Car]{\label{fig4:h}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/car_roc.pdf}}\\
\subfloat[Iris]{\label{fig4:i}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/iris_roc.pdf}}\quad
\subfloat[Seeds]{\label{fig4:j}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/seeds_roc.pdf}}\quad
\subfloat[Ecoli]{\label{fig4:k}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/roc/ecoli_roc.pdf}}\\
\caption{ROC curves of comparison and our model on all datasets.}
\label{fig:4}
\end{figure*}

% \begin{figure*}[htb]
% \centering
% \subfloat{\label{fig:a}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/breast_roc.pdf}}\quad
% \subfloat{\label{fig:b}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/blood-transfusion_roc.pdf}}\quad
% \subfloat{\label{fig:c}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/heart_roc.pdf}}\quad
% \subfloat{\label{fig:d}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/raisin_roc.pdf}}\\
% \subfloat{\label{fig:e}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/caesarian_roc.pdf}}\quad
% \subfloat{\label{fig:f}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/glass_roc.pdf}}\quad
% \subfloat{\label{fig:g}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/wine_roc.pdf}}\quad
% \subfloat{\label{fig:h}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/car_roc.pdf}}\\
% \subfloat{\label{fig:i}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/iris_roc.pdf}}\quad
% \subfloat{\label{fig:j}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/seeds_roc.pdf}}\quad
% \subfloat{\label{fig:k}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/ecoli_roc.pdf}}\\
% \caption{ROC curves of comparison and our model on all datasets.}
% \label{fig:3}
% \end{figure*}

\subsection{Statistical analysis} \label{statis}
In this section, we first evaluate the sensitivity of all hyper-parameters from MODNF on one binary dataset Raisin and one multi-classification dataset Iris. Then, we analyse the convergence of MODNF with BBO and BP on all of the datasets.

Our model contains three hyper-parameters: the number of dendrites $M$, synaptic scaling factor $\alpha_s$ and telodendron scaling factor $\alpha_t$. More precisely, $M$ can controls the structure of the model, then $\alpha_s$ and $\alpha_t$ can change the proportions in the synapses and telodendria, respectively. Fig. \ref{fig5:a} and \ref{fig5:b} shows the results when $M$ is varied from 4 to 20 with fixing $\alpha_s$ and $\alpha_t$. We could note that the best performance is achieved when $M$ is taken to be 8 on Raisin and 12 on Iris, which indicates a small $M$ can not sufficiently learn useful information from the data, while a large $M$ make optimization more difficult and are prone to overfitting. Fig. \ref{fig5:c} and \ref{fig5:d} present the ACC by traversing $\alpha_s$ and $\alpha_t$ on the interval of [0.1, 1, 5, 10, 25]. From the figure, the peak performance is achieved at $\alpha_s = 5$ and $\alpha_t = 1$.

\begin{figure}
\centering
\subfloat[$M$ on Raisin]{\label{fig5:a}\includegraphics[width=0.45\linewidth]{paper/figure/experiment/parameter/raisin_m.pdf}}\quad
\subfloat[$M$ on Iris]{\label{fig5:b}\includegraphics[width=0.45\linewidth]{paper/figure/experiment/parameter/iris_m.pdf}}\\
\subfloat[$\alpha^s$ on Raisin]{\label{fig5:c}\includegraphics[width=0.45\linewidth]{paper/figure/experiment/parameter/raisin_k.pdf}}\quad
\subfloat[$\alpha^s$ on Iris]{\label{fig5:d}\includegraphics[width=0.45\linewidth]{paper/figure/experiment/parameter/iris_k.pdf}}\\
\caption{The performance with three different parameters on the Raisin and Iris}
\label{fig:5}
\end{figure}

Fig. \ref{fig:6} appearances the scaled values of the cross entropy loss during optimizing. We can discover that the BBO algorithm can make MODNF converge with increasing number of iteration on all datasets, whereas as stated in \ref{evaluation}, BP has a hard time converging our model.

\begin{figure*}
\centering
\subfloat[Breast]{\label{fig6:a}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/breast_loss.pdf}}\quad
\subfloat[Blood transfusion]{\label{fig6:b}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/blood-transfusion_loss.pdf}}\quad
\subfloat[Heart]{\label{fig6:c}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/heart_loss.pdf}}\quad
\subfloat[Raisin]{\label{fig6:d}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/raisin_loss.pdf}}\\
\subfloat[Caesarian]{\label{fig6:e}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/caesarian_loss.pdf}}\quad
\subfloat[Glass]{\label{fig6:f}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/glass_loss.pdf}}\quad
\subfloat[Wine]{\label{fig6:g}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/wine_loss.pdf}}\quad
\subfloat[Car]{\label{fig6:h}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/car_loss.pdf}}\\
\subfloat[Iris]{\label{fig6:i}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/iris_loss.pdf}}\quad
\subfloat[Seeds]{\label{fig6:j}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/seeds_loss.pdf}}\quad
\subfloat[Ecoli]{\label{fig6:k}\includegraphics[width=0.22\linewidth]{paper/figure/experiment/loss/ecoli_loss.pdf}}\\
\caption{Convergence curves of MODNF under BBO and BP on all datasets.}
\label{fig:6}
\end{figure*}


==> paper/backup/introduction.tex <==
\section{Introduction}\label{intro}
\IEEEPARstart{N}{eurons} performed neurological functions are composed of somas and synapses, which are the basic structural and functional units of neural tissue. Neurons have the ability to perceive stimuli, integrate information and conduct impulses. Specifically, its electric potential changes when other neurons transmit chemicals to the current neuron, and it becomes excitatory until a threshold is reached, after which it begins to transmit chemicals to surrounding neurons. In 1943, McCulloch and Pitts abstracted this biological process and constructed the McCulloch-Pitts neuron which is the most commonly known neuron model at present \cite{mcculloch1943logical}. After that, Frank \cite{rosenblatt1961principles} used this model as a basis to propose the multi-layer perceptrons (MLP), which is now the basis of one of the most popular artificial neural networks. However, this model was criticized by Minsky and Papert for over-simplification and pointed out to have two fatal flaws \cite{marvin1969perceptrons}. On the one hand, no one can train the MLP perfectly enough due to the limitations in the single-layer perceptron. On the other hand, the single-layer perceptron have limited processing and cannot solve some easy problems such as nonlinear problems.

To address this issue, an algorithm called back-propagating (BP) was proposed to show a effective way for the training method of MLP \cite{rumelhart1986learning}. After that, Hornik et al. \cite{hornik1989multilayer} demonstrated that a deep neural network can be used to approximate any Borel measurable function regardless of the squashing function used as the activation function, and without limiting the size of the neural network. Therefore, artificial neural networks shine brilliantly in a wide range of fields such as image processing \cite{krizhevsky2017imagenet}, natural language processing (NLP) \cite{vaswani2017attention}, robotics \cite{he2016adaptive}.

In the meantime, there are many single neuron models dedicated to simulating the transmission process in neurons \cite{koch2000role} that have been proposed, such as pi-sigma models \cite{shin1991pi, ghosh1992efficient, fan2022convergence}, sigma-pi models \cite{gurney1992training, lenze1994make, heywood1995framework, neville2002transformations, weber2007self, long2007lp}, a single multiplicative neuron model \cite{yadav2007time, zhao2009pso, bas2016robust, kolay2023new}. Synaptic inputs in neurons are capable of not only linear reflections but also some nonlinear interactions when a synapses is in a specific location \cite{aguera2000can}. All of these frameworks structure this nonlinear aggregation pattern by constructing multiplication layers in the MP model. Because multiplication is the simplest and most basic nonlinear operation, it is a more reasonable choice to use this operation to implement the nonlinear function of artificial neurons. However, these neuronal models that rely on the McCulloch-Pitts model do not take into account the role of dendrites on neurons or express the biological information contained in dendrites. Therefore, spike-timing dependent plasticity (STDP) and branch-strength potentiation (BSP) method are united as the branch-specific plasticity neurons framework to implement the function of synapses and dendritic branching \cite{legenstein2011branch, bono2017modelling}. However, single nonlinear branch neurons do not have the functions that an exclusive OR (XOR) function have and it can only solve the XOR problem by adding inhibitory interneurons \cite{costa2011one}.


\gu{To further provide the capability for ANNs in modeling the non-linearity between synaptic input and output, todo et al. proposed the dendritic neuron model (DNM) that empowers the single multiplicative neuron models. Specifically, DNM employs the nonlinear function to model synapses, which makes synapses gain a nonlinear computational function and models the cell body and axon of neurons.}

morphology of a neuron
In addition, Gidons \cite{gidon2020dendritic}..
However, it still suffers from the major issue regarding the structural limitation: Since a single DNM is designed to have one single output, it cannot handle multi-output tasks. This great lowers the applications since the majority real-world tasks involve multiple outputs. Simply, there are two main approaches to constructing multi-output neuron framework for most neuronal units.


There are two main approaches to constructing a multi-output neuron framework for most neuronal units. First of all, a fully connected layer can be built directly to achieve the task of multiple outputs for some specific networks such as the MLP and the sigma-pi models. But only some models which treat neurons as the smallest unit can construct the fully connected layers. Furthermore, multiple neurons are stacked together when faced with multiple output tasks including the DNM \cite{kolay2023new, todo2014unsupervised, peng2023extension, geng2019multi}. It is undoubted that this method is the simplest and most immediate way to achieve the multiple output function of neuronal models. In contrast, most of neurons in an organism have some different branches at the end of the axon to connect to other neurons or somatic cells, although the number of axon in one neuron does not exceed one. In addition, this approach treats the different outputs as many independent individuals without any correlation, which is not conducive to the recognition of multiple classes of objects.


Recently, Gidon et al. discovered a calcium-mediated dendritic potential, called dendritic $\rm Ca^{2+}$ action potentials (dCaAPs), that can rely on neuronal dendrites to handle simple linearly inseparable problems and confirmed the idea that dendrite inputs and axon outputs can implement XOR functions by simulation experiments \cite{gidon2020dendritic}. Meanwhile, todo et al. designed the dendritic neuron model (DNM) considering the nonlinear relationship between synaptic input and output \cite{todo2014unsupervised}, and demonstrated the ability of the model to solve the XOR problem \cite{todo2019neurons}. Specifically, DNM employs a nonlinear function to model synapses, which makes synapses to gain a nonlinear computational function and models the cell body and axon of neurons. Hence, the DNM with synaptic non-linearity has been widely used in various fields and has achieved outstanding results \cite{ji2016approximate, gao2019dendritic, todo2019neurons, he2021seasonal, xu2021dendritic, gao2021fully, yu2022improving, ji2022competitive, peng2023extension}. However, the single DNM can only have a single output, so it cannot undertake multi-output tasks, such as multi-class classification tasks. There are two main approaches to constructing a multi-output neuron framework for most neuronal units. First of all, a fully connected layer can be built directly to achieve the task of multiple outputs for some specific networks such as the MLP and the sigma-pi models. But only some models which treat neurons as the smallest unit can construct the fully connected layers. Furthermore, multiple neurons are stacked together when faced with multiple output tasks including the DNM \cite{kolay2023new, todo2014unsupervised, peng2023extension, geng2019multi}. It is undoubted that this method is the simplest and most immediate way to achieve the multiple output function of neuronal models. In contrast, most of neurons in an organism have some different branches at the end of the axon to connect to other neurons or somatic cells, although the number of axon in one neuron does not exceed one. In addition, this approach treats the different outputs as many independent individuals without any correlation, which is not conducive to the recognition of multiple classes of objects.

In our study, we propose a multi-output dendritic neuron (MODN) in order to provide a framework to solve the above problem. Concisely, our model is dedicated to discriminating the signal received and integrated from dendrites by constructing a telodendron layer. In detail, we design a differential selection regulation in the soma layer in order to learn both the consensus information between different outputs, and the independent discriminative information used to distinguish each output. In addition, we utilize a nonlinear function in the telodendron layer to map the input information from the soma layer, so that a single neuron can also gain the ability to handle the XOR problem. Finally, it is necessary to ensure that the objective function is continuous due to the fact that the BP algorithm requires gradient of the objective model. Moreover, the BP algorithm can easily fall into a local optimal solution when optimizing a non-convex function. So we use some different heuristic algorithms to train the model with the aim of finding an effective optimization algorithm. The contributions of this study can be summarized as follows:

\begin{comment}
\begin{itemize}
	\item We first propose a new multi-output dendritic neuron (MODN) to solves the single output problem by constructing a new telodendron layer, which can perform different outputs depending on the different target cells;
	\item In the soma layer, a dendritic filtering method is used to prune out the redundant dendrites as a way to filter out the corresponding dendrities according to the target cells;
	\item To obtain an effective solution, several heuristic algorithms are used to optimize the parameters of the model.
\end{itemize}
\end{comment} 

\begin{itemize}
	\item We propose a novel framework that enables  dendritic neuron models to handle both single- and multi-output tasks in a unified formulation. 
 	\item We introduce a filtering matrix to adaptively select the desired dentrites for the downstream tasks.
   	\item We experimentally investigate the optimization strategies for our model with gradient-based and heuristic algorithms.  
        \item We report extensive experimental results against prior dendritic neuron models on classification tasks using 11 datasets to evaluate the effectiveness of our model.
\end{itemize}
        


The remainder of this paper is designed as follows. Section \uppercase\expandafter{\romannumeral2} introduces the structure and function of the DNM. Section \uppercase\expandafter{\romannumeral3} introduces the proposed in our study and its optimization algorithm. The experiments and discussion of the proposed method are shown in section \uppercase\expandafter{\romannumeral4}. In section \uppercase\expandafter{\romannumeral5}, a summary of our study is shown.


%	\item We first propose a new multi-output dendritic neuron (MODN) to solves the single output problem by constructing a new telodendron layer, which can perform different outputs depending on the different target cells;
%	\item In the soma layer, a dendritic filtering method is used to prune out the redundant dendrites as a way to filter out the corresponding dendrities according to the target cells;
%	\item To obtain an effective solution, several heuristic algorithms are used to optimize the parameters of the model.



==> paper/backup/methodology.tex <==
\section{Method}\label{method}
In this section, we detail our model $-$ Multi-output dendritic neuron model (MODN). Fig. \ref{fig:1} illustrates our model. Specifically, MODN consists of four layers: synaptic layer, dendrite layer, soma layer, and telodendron layer. We adopt the standard design of synaptic and dendrite layers in our MODN, following \cite{todo2014unsupervised, gao2019dendritic}. In designing the soma layer, 


\subsection{Multi-output dendritic neuron model}
In this section we reconstruct the structures in the DNM except synapses and dendrites. At first we eliminate the membrane layer, because directly adding the output from all dendrites would abandon the possibility of neurons learning dissensus information in the samples. As a superior substitute, we reconstruct the structure of the soma layer and design a extra telodendron layer to learn the representation information of different attributes in the sample, as shown in Fig. \ref{fig:1}.

\begin{figure*}[htb]
\begin{center}
\includegraphics[width=1.0\linewidth]{paper/figure/methodology/Fig1.pdf}
\end{center}
\caption{The illustration of transmission process in multi-output dendritic neuron.}
\label{fig:1}
\end{figure*}

\noindent \textbf{Preference filter.} We follow the synaptic layer and dendritic layer in the DNM model. This dendritic structure can convert the input to the output by different connected state synaptic nodes. In addition, a soft AND function is utilized to merge each input on the dendrites considering the interactions between the inputs. In our soma layer, we propose a binary preference matrix that is capable of meticulously dividing the dendrites as a way to generate different neural information. This filtering process can produce different neural signals depending on the number and the characteristics of the output target. Hence, the above process is defined as
\begin{equation}
\label{eq:eq5}
V=Z\times{\boldsymbol{P}},
\end{equation}
where $Z=[Z_{1},...,Z_{m},...,Z_{M}]$ and $V=[V_{1},...,V_{c},...,V_{C}]$ are the output from the dendrite layer and the soma layer, respectively. $\boldsymbol{P}\in{\{0,1\}}^{M\times C}$ represents a Boolean matrix learned by the network. The rows and columns in the filter correspond to all of dendrites and outputs. Each column in the matrix $\boldsymbol{P}$ directs the dendrites to synthesize information unique to one of outputs. And the filter can assign a different role to each dendrite. More explicitly, dendrites can be divided into three types depending on the state of the filter.
\begin{itemize}
        \item \textit{Inoperative dendrite.} This state is activated when all elements of a row in the matrix $\boldsymbol{P}$ equal to 0. Here, the dendrite does not influence the neuron because the signal generated by the dendrite corresponding to the column does not pass backward. 
        % This state is activated when there is only one value of 1 in a row of the matrix $\boldsymbol{P}$.
        \item \textit{Exclusive dendrite.} This state is activated when one of the row in the matrix $\boldsymbol{P}$ is an one-hot vector. It indicates that the dendrite in connection with this row captures some unique attributes from the data corresponding to the output of this column.
        \item \textit{Communal dendrite.} This state is activated when a row in the matrix $\boldsymbol{P}$ contains more than one element of 1. Here, the dendrite corresponding to this row is able to learn the joint features for the outputs with 1-valued elements in $\boldsymbol{P}$ in this row.
        
        
%        When all elements of a row in the matrix $\boldsymbol{P}$ equal to 0, it means that the signal generated by the dendrite corresponding to the column does not pass backward, that is to say, the dendrite does not produce any effects in the neuron.
%        \item \textit{Exclusive dendrite.}  When there is only one value of 1 in a row of the matrix $\boldsymbol{P}$, it indicates that the dendrite in connection with this row can acquire the unique information in the data corresponding to the output of this column.
%        \item \textit{Communal dendrite.} When a row in the matrix $\boldsymbol{P}$ contains more than one element of 1, the dendrite corresponding to this row is able to learn the consensus information between the outputs corresponding to these elements.
\end{itemize}
% In theory, the preference filter $\boldsymbol{P}$, which is learned from the optimization of the dendrite neuron, can adaptively categorize 
% any dendrite into these three types of dendrites. 

In theory, altering the preference filter $\boldsymbol{P}$, which is learned from the optimization of the dendrite neuron, can adaptively categorize any dendrite into these three activation styles. However, since the inoperative dendrite would block the behavior of the related dendrite in the neural transmission process, including this type of dendrite does not have any positive effect on the downstream task (e.g., classification), while increasing computational overhead. We thus exclude the inoperative dendrite in our implementation by appropriately designing the value of dendritic branches $M$. Consequently, we only include the exclusive dendrite and the communal dendrite in our model for further encoding efficiency.



%Under normal circumstances, the preference filter $\boldsymbol{P}$ is learned from the optimization of the dendrite neuron, which can adaptively induce the dendrites differentiation into the aforementioned specific dendrites, namely the exclusive dendrite and the communal dendrite, in theory. In addition to the two kinds of specific dendrites above, it is necessary to mention that the inoperative dendrite, since it will block the action of the related dendrite in the neural transmission process, is avoided by designing the reasonable value of dendritic branches $M$.

Specifically, our proposed preference filter is a generalized dendritic neuron model, which contains the case of stacking multiple original single dendritic neuron models. Due to such a beneficial property, the dendrites can be conveniently divided into $C$ completely independent groups by the preference filter $\boldsymbol{P}$, where only one possible state of the exclusive dendrite can exist. As such, each group of dendrites can be regarded as the dendrites in the corresponding single DNM model since they are all mutually independent. We thus regard this case as a MODN variant, and term it as MODN partition (MODNP), as shown in Fig. \ref{fig:2}.

In contrast, when the filter matrix $\boldsymbol{P}$ is all-ones matrix, it is trivial to derive that only one possible state of the communal dendrite can exist. To be more precise, the particular neuron possesses every dendrite of the ability to learn all attributes at the same time. The above special neuron with the all-ones preference filter is called MODN full (MODNF).

\begin{figure}[htb]
\centering
  \includegraphics[width=1\linewidth]{paper/figure/methodology/Fig2.pdf}
   \caption{The illustration of transformation between (a) MODNP and (b) DNMs. (Take three outputs and the value of $M$ is 6, for example.) } 
\label{fig:2}
\end{figure}


\noindent \textbf{Telodendron layer.} In nerve cells, axons are the output channels of neurons that can connect to one or more target cells. Some axons branch out and form telodendria at the end of each axon. In our model, we use the tanh function to map the different signals to the range from -1 to 1. The function of telodendron layer is written as
\begin{equation}
\label{eq:eq6}
R_{c}=\frac{e^{\alpha_{t}(\omega^{t}_{c}V_{c}-\theta^{t}_{c})}-e^{-\alpha_{t}(\omega^{t}_{c}V_{c}-\theta^{t}_{c})}}{e^{\alpha_{t}(\omega^{t}_{c}V_{c}-\theta^{t}_{c})}+e^{-\alpha_{t}(\omega^{t}_{c}V_{c}-\theta^{t}_{c})}},
\end{equation}
where $R_c$ $(c=1,...,C)$ means the output from the $c$-th telodendron layer. $\alpha_{t}$ denotes the telodendron scaling factor, similarly to the one in the synaptic layer. $\omega^{t}_{c}$ and $\theta^{t}_{c}$ are the weight and threshold from the $c$-th telodendron. Compared with the sigmoid function, the tanh in the telodendron layer can multiply the output value of the neuron in range of (-1, 1), which can improve more flexibility and potential discrimination in the transmission process between neurons or target cells.

\noindent \textbf{Target cell.} The target cell is a unit that is connected to the front neuron and have the function of receiving information from the front neuronal cell. In our proposed, our aim is to recognize the multiple class attributes of samples. As such, we utilize a softmax function as the target cell in our framework. We then adopt the (binary) cross entropy to measure the fitting degree of our model. The above two processes are mathematically fulfilled as
\begin{equation}
\label{eq:eq7}
O_{c}=\frac{e^{R_{c}}}{\sum_{c=1}^{C}e^{R_{c}}},
\end{equation}
\begin{equation}
\label{eq:eq8}
\mathcal{L}=-\frac{1}{N}\sum_{n=1}^{N}\sum_{c=1}^{C}\widehat{O}_{c}^{n}\log(O_{c}^{n}),
\end{equation}
where $O_{c}^{n}$ is the output probability that the $n$-th sample belongs of class $c$ and $\widehat{\cdot}$ is the ground truth of the corresponding sample.
\subsection{Optimization}
A prevalent selection for optimizing the network such as deep neural network is BP. However, the fact that $\boldsymbol{P}$ is discrete in its solution space makes it less feasible to directly take partial derivative and propagate the gradient. Hence, learning MODN requires other gradient-free techniques. To address this, we resort to heuristic algorithms to explore decent solutions within acceptable processing time. Specifically, we employ five types of heuristic algorithms to examine the performance: biogeography-based optimization (BBO) \cite{simon2008biogeography}, genetic algorithm (GA) \cite{simon2013evolutionary}, particle swarm optimization (PSO) \cite{eberhart1995new}, population-based incremental learning (PBIL) \cite{baluja1994population}, and evolutionary strategy (ES) \cite{engelbrecht2007computational}. 


%it is trivial to find that the undetermined matrix $\boldsymbol{P}$ is discrete in its solution space, which results in its partial derivative not existing. Hence, BP cannot be used to optimize the MODN but only the MODNP and MODNF with the certain matrix $P$. Hence, unlike MODNP and MODNF which can directly be optimized with BP, learning MODN requires gradient-free techniques. To address this, we resort to heuristic algorithms to explore decent solutions within acceptable processing time. Specifically, we employ five types of heuristic algorithms to examine the classification performance: biogeography-based optimization (BBO), genetic algorithm (GA), particle swarm optimization (PSO), population-based incremental learning (PBIL) and evolutionary strategy (ES). 

%For optimizing the MODN, we utilize five heuristic algorithms (HAs), which are biogeography-based optimization (BBO), genetic algorithm (GA), particle swarm optimization (PSO), population-based incremental learning (PBIL) and evolutionary strategy (ES). HAs are a cunning kind of algorithms designed by intuition and experience, which can provide a decent solution of an optimizing problem to be solved within an acceptable time, generally in a polynomial time.

For MODNP and MODNF, we simply utilize BP and derive the update of our model since $\boldsymbol{P}$ is pre-determined. By introducing the learning rate $\eta$ and using recursively the preceding round, the $(r+1)$-th $(r=1,...,R)$ round of update for $\omega^{s}_{ij}, \theta^{s}_{ij}, \omega^{t}_{c}$ and $\omega^{t}_{c}, $ can be formulated as: 
\begin{equation}
\label{eq:eq9}
w^{s}_{ij(r+1)}=w^{s}_{ij(r)}-\eta \nabla \mathcal{L}(w^{s}_{ij(r)}),
\end{equation}
\begin{equation}
\label{eq:eq10}
\theta^{s}_{ij(r+1)}=\theta^{s}_{ij(r)}-\eta \nabla \mathcal{L}(\theta^{s}_{ij(r)}),
\end{equation}
\begin{equation}
\label{eq:eq11}
w^{t}_{c(r+1)}=w^{t}_{c(r)}-\eta \nabla \mathcal{L}(w^{t}_{c(r)}),
\end{equation}
\begin{equation}
\label{eq:eq12}
\theta^{t}_{c(r+1)}=\theta^{t}_{c(r)}-\eta \nabla \mathcal{L}(\theta^{t}_{c(r)}),
\end{equation}
where $\nabla$ denotes the partial derivative operator. In particular, the partial derivatives of $\mathcal{L}$ with respect to $w_{t}$ and $\theta_{t}$ in Eqs. \ref{eq:eq11} and \ref{eq:eq12} can be respectively derived as:
\begin{equation}
\begin{aligned}
\label{eq:eq13}
\nabla \mathcal{L}(w^{t}_{c(r)})&= \frac{\partial\mathcal{L}}{\partial O_c}\frac{\partial O_c}{\partial R_c}\frac{\partial R_c}{\partial w^{t}_{c}}\\
&=\frac{\widehat{O}_{c}}{N}k_{t}V_{c}(O_{c}-1)(1-R_c^2),
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
\label{eq:eq14}
\nabla \mathcal{L}(\theta^{t}_{c(r)}) &= \frac{\partial\mathcal{L}}{\partial O_c}\frac{\partial O_c}{\partial R_c}\frac{\partial R_c}{\partial\theta^{t}_{c}}\\
&=\frac{\widehat{O}_{c}}{N}k_{t}(1-O_{c})(1-R_c^2),
\end{aligned}
\end{equation}
where $c$ refers to the 1-valued index in the corresponding groundtruth label. 


Since a different design of $\boldsymbol{P}$ results in varying filtering strategies, the update for MODNP and MODNF needs to be separately considered. For MODNP, the gradients regarding $w$ and $\theta$ can be calculated as
\begin{equation}
\begin{aligned}
\label{eq:eq15}
\nabla \mathcal{L}(w^{s}_{ij(r)}) = &\frac{\partial\mathcal{L}}{\partial O_c}\frac{\partial O_c}{\partial R_c}\frac{\partial R_c}{\partial V_c}\frac{\partial V_c}{\partial Z_{j}}\frac{\partial Z_{j}}{\partial Y_{ij}}\frac{\partial Y_{ij}}{\partial w^{s}_{ij}}\\
=&\frac{\widehat{O}_{c}}{N}k_{t}w^{t}_{c}kx_{ij}(O_{c}-1)(1-R_c^2)p_{jc}\\
&(\prod_{q=1(q \neq i)}^{D}Y_{qj})Y_{ij}(Y_{ij}-1),
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
\label{eq:eq16}
\nabla \mathcal{L}(\theta^{s}_{ij(r)})=&\frac{\partial\mathcal{L}}{\partial O_c}\frac{\partial O_c}{\partial R_c}\frac{\partial R_c}{\partial V_c}\frac{\partial V}{\partial Z_{j}}\frac{\partial Z_{j}}{\partial Y_{ij}}\frac{\partial Y_{ij}}{\partial\theta^{s}_{ij}}\\
=&\frac{\widehat{O}_{c}}{N}k_{t}w^{t}_{c}k(O_{c}-1)(1-R_c^2)p_{jc}\\
&(\prod_{q=1(q \neq i)}^{D}Y_{qj})Y_{ij}(1-Y_{ij}),
\end{aligned}
\end{equation}
where $p_{jc}$ is an element of the $j$-the row and the $c$-the column of the $\boldsymbol{P}$; for MODNF, the gradients regarding $w$ and $\theta$ can be measured via
\begin{equation}
\begin{aligned}
\label{eq:eq17}
\nabla \mathcal{L}(w^{s}_{ij(r)}) = &\frac{\partial\mathcal{L}}{\partial O_c}O_{c}(\frac{\partial R_c}{\partial w^{s}_{ij}}-\sum_{s=1}^{C}O_{s}\frac{\partial R_s}{\partial w^{s}_{ij}})\\
=&\frac{\widehat{O}_{c}}{N}(\frac{\partial R_c}{\partial w^{s}_{ij}}-\sum_{s=1}^{C}O_{s}\frac{\partial R_s}{\partial w^{s}_{ij}}),
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
\label{eq:eq18}
\nabla \mathcal{L}(\theta^{s}_{ij(r)}) = &\frac{\partial\mathcal{L}}{\partial O_c}O_{c}(\frac{\partial R_c}{\partial \theta^{s}_{ij}}-\sum_{s=1}^{C}O_{s}\frac{\partial R_s}{\partial \theta^{s}_{ij}})\\
=&\frac{\widehat{O}_{c}}{N}(\frac{\partial R_c}{\partial \theta^{s}_{ij}}-\sum_{s=1}^{C}O_{s}\frac{\partial R_s}{\partial \theta^{s}_{ij}}),
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
\label{eq:eq19}
\frac{\partial\mathcal{R}_{s}}{\partial w^{s}_{ij}} = &\frac{\partial R_{s}}{\partial V_{s}}\frac{\partial V_{s}}{\partial Z_{j}}\frac{\partial Z_{j}}{\partial Y_{ij}}\frac{\partial Y_{ij}}{\partial w^{s}_{ij}}(s = 1, ..., C)\\
=&k_{t}w^{t}_{s}kx_{i}(1-R_s^2)\\
&(\prod_{q=1(q \neq i)}^{D}Y_{qj})Y_{ij}(Y_{ij}-1),
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
\label{eq:eq20}
\frac{\partial\mathcal{R}_{s}}{\partial \theta^{s}_{ij}} = &\frac{\partial R_{s}}{\partial V_{s}}\frac{\partial V_{s}}{\partial Z_{j}}\frac{\partial Z_{j}}{\partial Y_{ij}}\frac{\partial Y_{ij}}{\partial \theta^{s}_{ij}}(s = 1, ..., C)\\
=&k_{t}w^{t}_{s}k(1-R_s^2)\\
&(\prod_{q=1(q \neq i)}^{D}Y_{qj})Y_{ij}(1-Y_{ij}).
\end{aligned}
\end{equation}

Note that we modify all zero-valued $Y$ (we treat $Y$ as 0 when $Y$ is smaller than $10^{-9}$) to 1 to prevent the phenomenon of ``dendrite dying''. That is, when more than one connection condition of synaptic node falls into the \textit{Unvarying 0 state}, the gradient in the corresponding dentrite would always be reduced to 0 and never get updated. The detailed 
derivation is given in \textbf{Proposition} \ref{T1}.

\begin{theorem}\label{T1}
    There exists a non-zero gradient in the BP optimization process, if and only if the number of zero-valued independent variables is at most one in Eq. \ref{eq:eq2}.
\end{theorem}

\begin{proof}
    \textit{The proof for} \textbf{Proposition} \ref{T1} \textit{is as follows. Here, we assume the following multiplication:}     
    \begin{equation}
    \label{eq:eq21}
        z=\prod_{i=1}^{D}y_{i}
    \end{equation}
    \textit{by omitting the subscript $j$ in Eq. \ref{eq:eq2} for simplicity without the loss of generality. With a minor abuse of notation, we define the variable set $Y=\{y_1,\cdots,y_D\}$. By taking the partial derivative for Eq. \ref{eq:eq21} with respect to $y_p\in Y$, we obtain}     
    \begin{equation}
    \label{eq:eq22}
        \frac{\partial z}{\partial y_p}=\prod_{i=1,  i\neq p}^{D}y_{i}.
    \end{equation}
    \textit{Given the number of zero-valued variables in $Y$, the following three cases can be discussed during the model update:}
    \begin{itemize}
        \item     \textit{CASE 1: If $\forall y_p\in Y, y_{p}\neq 0$ holds, then Eq. \ref{eq:eq22} is a non-zero value. Therefore, the network can be successfully updated.}
        
        \item   \textit{CASE 2: If at least two variables in $Y$ are 0 (e.g., $y_{p}$ and $y_{q}$), then the partial derivatives with respect to all variables are always be 0 despite the update being performed, because the partial derivatives should always include at least one or both of $y_{p}$ and $y_{q}$. Therefore, the "dendrite dying" issue is triggered and the network fails to update. }
        
        \item   \textit{CASE 3: If one and only one variable (e.g., $y_{p}$) is 0, then the partial derivatives with respect to the remaining variables in Y (i.e., $\{y_1,\cdots,y_{p-1},y_{p+1}, \cdots, y_D\}$) are also 0. Ideally, because the partial derivative with respect to $y_{p}$ is still a non-zero value, all of variables will be non-zero values in the next round of update. However, due to the chain rule, we need multiply by the partial derivative of Eq. \ref{eq:eq1} in later calculation so that $y_{p}$ is still contained in the gradient of $\mathcal{L}$ with respect to $w^{s}_{ij(r)}$ and $\theta^{s}_{ij(r)}$. As thus, the network is still unable to successfully updated since CASE 3 is equivalent to CASE 2.}
    \end{itemize}
%    \textit{Thus, for all possible cases, we should make sure at most one zero-valued variable in the Eq. \ref{eq:eq21} for stably updating model with BP.}
\end{proof}



To nonetheless tackle this issue, we simply set $Y_{qj}$ to 1 to enable back-propagation without manually imposing additional constraints. We also adopt the heuristic algorithms to optimize the MODNP and MODNF (see in Sec. \ref{experiments}).


==> paper/backup/relatedwork.tex <==
\section{Preliminaries}\label{relate}
DNM is modeled into a synaptic layer, a dendrite layer, membrane layer and a soma layer to simulate the internal function of neurons, especially the nonlinearity on dendrites. Generally, both of synaptic and soma layers exploit nonlinear activation functions to constitute a single-input and single-output node. The multiplicative and additive rules are applied to the dendrite and membrane layers to approximate the AND and OR functions, respectively.

\noindent \textbf{Synaptic Layer.} Synapses are channels through which information is exchanged within the central nervous system or between the central nervous system and other parts of the body, such as receptors. In general, neurons communicate with target cells dependent on the release and reception of neurotransmitters. Binding of the postsynaptic membrane to neurotransmitters generally results in transmembrane currents. Depolarized transmembrane currents result in excitatory postsynaptic potentials and hyperpolarized transmembrane currents result in inhibitory postsynaptic potentials. A sigmoid function with a translation and symmetry transformations is used to model this process. Assume the set of samples after normalization is $\boldsymbol{X}=[X^{1},...,X^{n},...,X^{N}]\in{R^{D\times{N}}}$. Assume further that the $n$-th single sample is $X^{n}=[x_{1}^{n},...,x_{d}^{n},...,x_{D}^{n}]^{T}$. Then the nonlinear mapping of the synaptic layer to the $n$-th sample (the superscript $n$ is dropped for brevity in all the following equations and figures) is given by
\begin{equation}
\label{eq:eq1}
Y_{ij}=\frac{1}{1+e^{-\alpha_{s} (\omega^{s}_{ij}x_{i}-\theta^{s}_{ij})}},
\end{equation}
where $x_{i}$ is the $i$-th $(i=1,...,D)$ input to the dendrite after normalization, and $y_{ij}$ is the output of the $i$-th synaptic node on the $j$-th $(j=1,...,M)$ dendrite. The learnable parameter pair ($\omega^{s}_{ij}$, $\theta^{s}_{ij}$), which respectively denotes the weights and thresholds, jointly controls the connections states of synaptic. $\alpha_{s}$, termed as synaptic scaling factor, is a hyperparameter to indicate the scaling strength. Eq. \ref{eq:eq1} computes the output of $i$-th synaptic on the $j$-th dendrite. Synaptic nodes on the dendrites respond accordingly to the input signal through these learnable parameters. Specifically, connection conditions can be divided into four types, including the excitatory state, the inhibitory state, the unvarying 0 state and the unvarying 1 state.

\begin{itemize}
	% \item \textbf{Excitatory state.} The input signal has a direct correlation with the output signal at this state node.
	% \item \textbf{Inhibitory state.}
        % \item \textbf{Unvarying 0 state.}
        % \item \textbf{Unvarying 1 state.}
        \item \textit{Excitatory state.} The input signal has a direct correlation with the output signal at this state node. This state is activated when both $\omega^{s}_{ij}$ and $\theta^{s}_{ij}$ are greater than 0 and $\omega^{s}_{ij}$ is greater than $\theta^{s}_{ij}$.
        \item \textit{Inhibitory state.}  The input signal has an inverse correlation with the output signal at this state node. This state is activated when both $\omega^{s}_{ij}$ and $\theta^{s}_{ij}$ are less than 0 and $\omega^{s}_{ij}$ is less than $\theta^{s}_{ij}$.
        \item \textit{Unvarying 0 state.} The output is 0 for any input between 0 and 1 at this state node. This state is activated when both $\omega^{s}_{ij}$ and $\theta^{s}_{ij}$ are greater than 0 and $\theta^{s}_{ij}$ is greater than $\omega^{s}_{ij}$, or $\theta^{s}_{ij}$ is greater than 0 but $\omega^{s}_{ij}$ is less than 0.
        \item \textit{Unvarying 1 state.} The output is 1 for any input between 0 and 1 at this state node. This state is activated when both $\omega^{s}_{ij}$ and $\theta^{s}_{ij}$ are less than 0 and $\theta^{s}_{ij}$ is less than $\omega^{s}_{ij}$, or $\theta^{s}_{ij}$ is less than 0 but $\omega^{s}_{ij}$ is greater than 0.
\end{itemize}

\noindent \textbf{Dendrite Layer.} Dendrites integrate nonlinearly and transmit the received excitatory and inhibitory inputs at the synapse to the cell membrane \cite{liu2004local, london2005dendritic}. However, it is very difficult to model the dendritic structure with the complex structure and abundant ion channels. Therefore, DNM simplifies this process by using a simple nonlinear algorithm. Specifically, a multiplicative function is used to implement the AND function between synapses as follow
\begin{equation}
\label{eq:eq2}
Z_{j}=\prod_{i=1}^{D}Y_{ij},
\end{equation}
where $Z_{j}$ means the output of the $j$-th branch.

\noindent \textbf{Membrane Layer.} The OR operation is utilized at the membrane layer different from the AND operation at the dendrite layer, i.e.,
\begin{equation}
\label{eq:eq3}
V=\sum_{j=1}^{M}Z_{j},
\end{equation}
where $V$ represent the output from the membrane layer, which is also the input of the soma layer.

\noindent \textbf{Soma Layer.} The soma, or the neuronal cell body, is the information processing centers of neurons. The electrical signals received from other neurons on the previous layers are eventually collected in the soma for subsequent processing. A sigmoid function is used to model this process with the following equation.
\begin{equation}
\label{eq:eq4}
O=\frac{1}{1+e^{-\alpha_{o}(v-\theta_{o})}}.
\end{equation}
where $o$ represent the final output from the neuron. In addition, $\alpha_{o}$ and $\theta_{o}$ are two positive hyperparameters to yield the output of model.

DNM can respond to the input data through the above process and has the effectiveness in many tasks such as classification, prediction and approximation. However, it suffers from the following two obvious disadvantages. (i): DNM cannot learn different information from the same sample due to the fact that the simple and crude strategy. (ii): The soma function is so monotonous that cannot take the value of previous layer for different targets.
